Prediction and Quantification of Individual Athletic Performance

We provide scientific foundations for athletic performance prediction on an individual level, exposing the phenomenology of individual athletic running performance in the form of a low-rank model dominated by an individual power law. We present, evaluate, and compare a selection of methods for prediction of individual running performance, including our own, \emph{local matrix completion} (LMC), which we show to perform best. We also show that many documented phenomena in quantitative sports science, such as the form of scoring tables, the success of existing prediction methods including Riegel's formula, the Purdy points scheme, the power law for world records performances and the broken power law for world record speeds may be explained on the basis of our findings in a unified way.

==> tables/tex_table_relative_time.tex <==
\begin{tabular}{cccc|cc|cccc|cc|cc}
&&&\multicolumn{1}{c}{}& \multicolumn{2}{c}{\vtop{\hbox{\strut }\hbox{\strut Baselines}}} & \multicolumn{4}{c}{\vtop{\hbox{\strut Performance }\hbox{\strut Predictors}}} & \multicolumn{2}{c}{\vtop{\hbox{\strut State of art}\hbox{\strut Matrix Completion}}} & \multicolumn{2}{c}{\vtop{\hbox{\strut Proposed}\hbox{\strut Method}}} \\ 
\rotatebox{90}{evaluation} & \rotatebox{90}{percentiles} & \rotatebox{90}{no.events} & \rotatebox{90}{data type} & \rotatebox{90}{r.mean} & \rotatebox{90}{k-NN} & \rotatebox{90}{ind.power} & \rotatebox{90}{riegel} & \rotatebox{90}{power l.} & \rotatebox{90}{purdy} & \rotatebox{90}{nucl.n.} & \rotatebox{90}{EM} & \rotatebox{90}{LMC r1} & \rotatebox{90}{LMC r2} \\ \hline 
log time & 0-95 & 3 & best & 0.13 & 0.119 & 0.0959 & 0.0973 & 0.0964 & 0.0596 & 0.178 & 0.056 & 0.0569 & 0.0499 \\ 
&&& & $\pm$0.003 & $\pm$0.003 & $\pm$0.003 & $\pm$0.007 & $\pm$0.007 & $\pm$0.003 & $\pm$0.01 & $\pm$0.003 & $\pm$0.002 & $\pm$0.002 \\ 
log time & 0-95 & 3 & random & 0.136 & 0.121 & 0.0874 & 0.0907 & 0.0895 & 0.0585 & 0.196 & 0.0544 & 0.055 & 0.0461 \\ 
&&& & $\pm$0.003 & $\pm$0.002 & $\pm$0.003 & $\pm$0.003 & $\pm$0.003 & $\pm$0.003 & $\pm$0.01 & $\pm$0.002 & $\pm$0.002 & $\pm$0.002 \\ 
log time & 0-95 & 4 & best & 0.123 & 0.118 & 0.075 & 0.0782 & 0.0785 & 0.0566 & 0.117 & 0.0525 & 0.0522 & 0.0455 \\ 
&&& & $\pm$0.003 & $\pm$0.002 & $\pm$0.002 & $\pm$0.003 & $\pm$0.003 & $\pm$0.002 & $\pm$0.008 & $\pm$0.003 & $\pm$0.002 & $\pm$0.002 \\ 
log time & 0-25 & 3 & best & 0.0559 & 0.053 & 0.076 & 0.0668 & 0.0704 & 0.0406 & 0.158 & 0.0377 & 0.0402 & 0.0302 \\ 
&&& & $\pm$0.001 & $\pm$0.001 & $\pm$0.002 & $\pm$0.002 & $\pm$0.002 & $\pm$0.001 & $\pm$0.01 & $\pm$0.001 & $\pm$0.001 & $\pm$0.001 \\ 
\end{tabular}

==> tables/tex_table_rmae.tex <==
\begin{tabular}{cccc|cc|cccc|cc|cc}
&&&\multicolumn{1}{c}{}& \multicolumn{2}{c}{\vtop{\hbox{\strut Generic}\hbox{\strut Baselines}}} & \multicolumn{4}{c}{\vtop{\hbox{\strut State of art}\hbox{\strut Performance Predictors}}} & \multicolumn{2}{c}{\vtop{\hbox{\strut State of art}\hbox{\strut Matrix Completion}}} & \multicolumn{2}{c}{\vtop{\hbox{\strut Proposed}\hbox{\strut Method: LMC}}} \\ 
\rotatebox{90}{evaluation} & \rotatebox{90}{percentiles} & \rotatebox{90}{no.events} & \rotatebox{90}{data type} & \rotatebox{90}{r.mean} & \rotatebox{90}{k-NN} & \rotatebox{90}{\parbox{1cm}{individual\\power law}} & \rotatebox{90}{riegel} & \rotatebox{90}{power law} & \rotatebox{90}{purdy} & \rotatebox{90}{\parbox{1cm}{nuclear\\norm}} & \rotatebox{90}{EM} & \rotatebox{90}{\parbox{1cm}{LMC\\rank 1}} & \rotatebox{90}{\parbox{1cm}{LMC\\rank 2}} \\ \hline 
log time & 0-95 & 3 & best & 0.0184 & 0.0167 & 0.014 & 0.0128 & 0.0126 & 0.00764 & 0.0217 & 0.007 & 0.00737 & \bf 0.00585 \\ 
&&& & $\pm$0.0005 & $\pm$0.0004 & $\pm$0.0005 & $\pm$0.0005 & $\pm$0.0005 & $\pm$0.0003 & $\pm$0.002 & $\pm$0.0003 & $\pm$0.0003 & \bf $\pm$0.0002 \\ 
normalized & 0-95 & 3 & best & 0.106 & 0.0954 & 0.0669 & 0.0654 & 0.0647 & 0.042 & 0.0876 & 0.0384 & 0.0397 & \bf 0.0333 \\ 
&&& & $\pm$0.002 & $\pm$0.002 & $\pm$0.002 & $\pm$0.002 & $\pm$0.002 & $\pm$0.001 & $\pm$0.005 & $\pm$0.001 & $\pm$0.001 & \bf $\pm$0.001 \\ 
speed & 0-95 & 3 & best & 0.106 & 0.098 & 0.0732 & 0.0677 & 0.0669 & 0.0428 & 0.433 & 0.0391 & 0.0408 & \bf 0.0341 \\ 
&&& & $\pm$0.003 & $\pm$0.003 & $\pm$0.003 & $\pm$0.002 & $\pm$0.002 & $\pm$0.001 & $\pm$0.2 & $\pm$0.001 & $\pm$0.001 & \bf $\pm$0.001 \\ 
log time & 0-95 & 3 & random & 0.0196 & 0.0171 & 0.0135 & 0.0127 & 0.0125 & 0.0073 & 0.0249 & 0.00664 & 0.00704 & \bf 0.00557 \\ 
&&& & $\pm$0.0005 & $\pm$0.0004 & $\pm$0.0005 & $\pm$0.0004 & $\pm$0.0004 & $\pm$0.0003 & $\pm$0.002 & $\pm$0.0003 & $\pm$0.0003 & \bf $\pm$0.0002 \\ 
normalized & 0-95 & 3 & random & 0.112 & 0.0982 & 0.0635 & 0.0651 & 0.0642 & 0.041 & 0.098 & 0.0373 & 0.0381 & \bf 0.0318 \\ 
&&& & $\pm$0.002 & $\pm$0.002 & $\pm$0.002 & $\pm$0.002 & $\pm$0.002 & $\pm$0.001 & $\pm$0.006 & $\pm$0.001 & $\pm$0.001 & \bf $\pm$0.001 \\ 
speed & 0-95 & 3 & random & 0.114 & 0.102 & 0.0682 & 0.0667 & 0.0657 & 0.0415 & 0.503 & 0.0381 & 0.039 & \bf 0.0323 \\ 
&&& & $\pm$0.003 & $\pm$0.003 & $\pm$0.002 & $\pm$0.002 & $\pm$0.002 & $\pm$0.001 & $\pm$0.1 & $\pm$0.001 & $\pm$0.001 & \bf $\pm$0.001 \\ 
log time & 0-95 & 4 & best & 0.0178 & 0.0169 & 0.0116 & 0.0102 & 0.0102 & 0.00747 & 0.0116 & 0.00626 & 0.00661 & \bf 0.0054 \\ 
&&& & $\pm$0.0005 & $\pm$0.0004 & $\pm$0.0005 & $\pm$0.0004 & $\pm$0.0003 & $\pm$0.0003 & $\pm$0.0008 & $\pm$0.0002 & $\pm$0.0002 & \bf $\pm$0.0002 \\ 
log time & 0-25 & 3 & best & 0.00781 & 0.00755 & 0.0129 & 0.00979 & 0.0103 & 0.00604 & 0.018 & 0.00535 & 0.00586 & \bf 0.00414 \\ 
&&& & $\pm$0.0002 & $\pm$0.0002 & $\pm$0.0006 & $\pm$0.0004 & $\pm$0.0004 & $\pm$0.0002 & $\pm$0.002 & $\pm$0.0002 & $\pm$0.0002 & \bf $\pm$0.0001 \\ 
\end{tabular}
